Safe and Private Forward-Trading Platform for Transactive Microgrids

Transactive microgrids have emerged as a transformative solution for the problems faced by distribution system operators due to an increase in the use of distributed energy resources and rapid growth in renewable energy generation. Transactive microgrids are tightly coupled cyber and physical systems, which require resilient and robust financial markets where transactions can be submitted and cleared, while ensuring that erroneous or malicious transactions cannot destabilize the grid. In this paper, we introduce TRANSAX, a novel decentralized platform for transactive microgrids. TRANSAX enables participants to trade in an energy futures market, which improves efficiency by finding feasible matches for energy trades, reducing the load on the distribution system operator. TRANSAX provides privacy to participants by anonymizing their trading activity using a distributed mixing service, while also enforcing constraints that limit trading activity based on safety requirements, such as keeping power flow below line capacity. We show that TRANSAX can satisfy the seemingly conflicting requirements of efficiency, safety, and privacy, and we demonstrate its performance using simulation results

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}

==> archive/contributions.tex <==

 We present the design of \platform, a novel transactive energy platform that meets all four requirements. We build on and integrate our past work in this area \cite{Laszka17,transax,eisele2018solidworx}, introduce novel extensions and analysis for privacy, and present a new GridLAB-D \cite{chassin2008gridlab} based testbed. \change{The outline is as follows}{}.
\iAron{Mention somewhere here that we build TRANSAX on a distributed ledger platform with smart contract capabilities (just 2-3 lines on what this means).}

\iAron{Just present contributions first, not paper organization. We can reference section at the end of sentences, e.g., (Section \ref{sec:approach}).}
\iScott{I like the way it is because it makes it easier to find where the contributions are in the paper.}
Section \ref{sec:approach} details the of the formalization of our trading approach, including extensions to enable futures markets and privacy groups. The key contribution of this formalization is to provide privacy while enforcing safety constraints through the use of energy assets, groups, and safety constraints. Note that providing either alone is not difficult, the challenge appears when satisfying both. Our formalization also allows the prosumers to trade efficiently by enabling them to specify production and consumption offers with temporal flexibility, and energy trading problem is cast as a linear program which can be solved efficiently.

\iAron{Same, let's just present contributions (perhaps more concisely).}
\iScott{Contrary to this this comment, your earlier comment suggested making the introduction longer.}
In Section \ref{sec:components}, we discuss the components used to enable the formalization. The key contributions here are resilience, the enforcement of the safety constraints and other rules through the use of a smart contract, our hybrid solver architecture which combines the trustworthiness of a distributed ledger with the efficiency of conventional computation platforms for solving the linear program, and privacy-preserving billing which enables prosumers to disclose their trades to their smart meters in a trustworthy way, which can be used to limit the information that the DSO receives. 

\iAron{Let's provide full outline: mention Section 2 and 3 briefly in this paragraph (i.e., one sentence each).}
In Section \ref{sec:protocol}, we describe how the components interact to provide the energy trading functionality. Section \ref{sec:analysis}  provides analysis to show how the architecture meets the requirements presented above, and discuss the tradeoffs between privacy and trading efficiency. In Section \ref{sec:experimental}, we share the integrated testbed we are developing that uses GridLAB-D \cite{chassin2008gridlab} to simulate a transactive energy microgrid. Section \ref{sec:related} gives an overview of related work. In  Section \ref{sec:conclusion}, we present our conclusions.

==> archive/testbed-figs.tex <==
\begin{figure}
        \centering
        \begin{subfigure}{.49\textwidth}
            \input{figs/horizon-fig.tex}
            \vspace{-.5cm}
            \caption{Memory consumption and energy traded during a single interval of the simulation for various values of $T_{h}$ using the CPLEX solver.}
            \label{fig:loahNrgMEM}
        \end{subfigure}
        \vspace{.5cm}
        \hfill
        \begin{subfigure}{.49\textwidth}
            \input{figs/solveTime-fig.tex}
            \caption{\textit{Solve} time is how long it took the solver to find a solution to the energy trading problem. \textit{Solve and Submit} time is how long to took to find the solution and submit it to the smart contract.}
            \label{fig:solve}
        \end{subfigure}
        \vspace{.5cm}
        \begin{subfigure}{.49\textwidth}
            % \includegraphics[width=\textwidth]{figs/substn}
            \input{figs/substn-fig.tex}
            \caption{Substation load with and without TRANSAX.}
            \label{fig:substn}
        \end{subfigure}
        \hfill
        \begin{subfigure}{.49\textwidth}
            % \includegraphics[width=\textwidth]{figs/chargeLvl.png}
            \input{figs/chargeLvl-fig.tex}
            \caption{Average battery charge level.}
            \label{fig:chargeLvl}
        \end{subfigure}
        % \caption{}
    % \end{figure}
    % \begin{figure}
        % \centering
        \begin{subfigure}{.49\textwidth}
            % \includegraphics[width=\textwidth, trim=0 0.8cm 0 1.1cm, clip]{figs/powerTraded.png}
            \input{figs/powerTraded-fig.tex}
            \caption{Green: sum of all production offers for each interval. Red: negative sum of all consumption offers for each interval. Blue: sum of all energy traded in each interval, whose maximum value is the minimum of the production and consumption offers.}
            \label{fig:powerTraded}
        \end{subfigure}
        \hfill
        \begin{subfigure}{.49\textwidth}
            \input{figs/solar-fig.tex}
            % \includegraphics[width=\textwidth, trim=0 0.8cm 0 1cm, clip]{figs/solar.png}
            \caption{Yellow: simulated solar profile. Purple: simulated battery charge level. Orange: simulated energy traded. Blue: total energy trades recorded in the market.}
            \label{fig:soloar}
        \end{subfigure}
        %
    \end{figure}

==> figs/viewport-fig.tex <==
\begin{figure*}\scalebox{.5}{
    \centering
        \begin{overpic}[grid, tics=1,unit=1cm,scale=1]
        {figs/grid-fig.pdf}\label{fig:viewport}
        \end{overpic}{}}
    \caption{use overpic to get dimensions}
    \label{fig:my_label}
\end{figure*}{}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth, viewport=0.5cm 0.5cm 19.5cm 21cm,clip] {figs/grid-fig.pdf}
    \caption{use viewport to get size}
    \label{fig:FSM}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth, trim=.5 0.5cm 0.5cm 0.5cm,clip] {figs/grid-fig.pdf}
    \caption{use trim to get size}
    \label{fig:FSM}
\end{figure}
